Constrained multi-fidelity Bayesian optimization with automatic stop condition

Bayesian optimization (BO) is increasingly employed in critical applications to find the optimal design with minimal cost. While BO is known for its sample efficiency, relying solely on costly high-fidelity data can still result in high costs. This is especially the case in constrained search spaces where BO must not only optimize but also ensure feasibility. A related issue in the BO literature is the lack of a systematic stopping criterion. To solve these challenges, we develop a constrained cost-aware multi-fidelity BO (CMFBO) framework whose goal is to minimize overall sampling costs by utilizing inexpensive low-fidelity sources while ensuring feasibility. In our case, the constraints can change across the data sources and may be even black-box functions. We also introduce a systematic stopping criterion that addresses the long-lasting issue associated with BO's convergence assessment. Our framework is publicly available on GitHub through the GP+ Python package and herein we validate it's efficacy on multiple benchmark problems.

==> Ref.tex <==


@article{brochu2010tutorial,
  title={A tutorial on Bayesian optimization of expensive cost functions, with application to active user modeling and hierarchical reinforcement learning},
  author={Brochu, Eric and Cora, Vlad M and De Freitas, Nando},
  journal={arXiv preprint arXiv:1012.2599},
  year={2010}
}



@inproceedings{couckuyt2022bayesian,
  title={Bayesian optimization: tutorial},
  author={Couckuyt, Ivo and Gonzalez, Sebastian Rojas and Branke, Juergen},
  booktitle={Proceedings of the Genetic and Evolutionary Computation Conference Companion},
  pages={843--863},
  year={2022}
}



@article{shu2021multi,
  title={A multi-fidelity Bayesian optimization approach based on the expected further improvement},
  author={Shu, Leshi and Jiang, Ping and Wang, Yan},
  journal={Structural and Multidisciplinary Optimization},
  volume={63},
  pages={1709--1719},
  year={2021},
  publisher={Springer}
}


@article{tran2020smf,
  title={sMF-BO-2CoGP: A sequential multi-fidelity constrained Bayesian optimization framework for design applications},
  author={Tran, Anh and Wildey, Tim and McCann, Scott},
  journal={Journal of Computing and Information Science in Engineering},
  volume={20},
  number={3},
  year={2020},
  publisher={American Society of Mechanical Engineers Digital Collection}
}

@inproceedings{takeno2020multi,
  title={Multi-fidelity Bayesian optimization with max-value entropy search and its parallelization},
  author={Takeno, Shion and Fukuoka, Hitoshi and Tsukada, Yuhki and Koyama, Toshiyuki and Shiga, Motoki and Takeuchi, Ichiro and Karasuyama, Masayuki},
  booktitle={International Conference on Machine Learning},
  pages={9334--9345},
  year={2020},
  organization={PMLR}
}



@article{zhang2021multi,
  title={Multi-fidelity deep neural network surrogate model for aerodynamic shape optimization},
  author={Zhang, Xinshuai and Xie, Fangfang and Ji, Tingwei and Zhu, Zaoxu and Zheng, Yao},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={373},
  pages={113485},
  year={2021},
  publisher={Elsevier}
}
@article{li2022line,
  title={On-line transfer learning for multi-fidelity data fusion with ensemble of deep neural networks},
  author={Li, Zengcong and Zhang, Shu and Li, Hongqing and Tian, Kuo and Cheng, Zhizhong and Chen, Yan and Wang, Bo},
  journal={Advanced Engineering Informatics},
  volume={53},
  pages={101689},
  year={2022},
  publisher={Elsevier}
}

@article{sarkar2019multifidelity,
  title={Multifidelity and multiscale Bayesian framework for high-dimensional engineering design and calibration},
  author={Sarkar, Soumalya and Mondal, Sudeepta and Joly, Michael and Lynch, Matthew E and Bopardikar, Shaunak D and Acharya, Ranadip and Perdikaris, Paris},
  journal={Journal of Mechanical Design},
  volume={141},
  number={12},
  pages={121001},
  year={2019},
  publisher={American Society of Mechanical Engineers}
}




@article{picheny2013quantile,
  title={Quantile-based optimization of noisy computer experiments with tunable precision},
  author={Picheny, Victor and Ginsbourger, David and Richet, Yann and Caplin, Gregory},
  journal={Technometrics},
  volume={55},
  number={1},
  pages={2--13},
  year={2013},
  publisher={Taylor \& Francis}
}




@article{sun2022correlated,
  title={Correlated multi-objective multi-fidelity optimization for HLS directives design},
  author={Sun, Qi and Chen, Tinghuan and Liu, Siting and Chen, Jianli and Yu, Hao and Yu, Bei},
  journal={ACM Transactions on Design Automation of Electronic Systems (TODAES)},
  volume={27},
  number={4},
  pages={1--27},
  year={2022},
  publisher={ACM New York, NY}
}

@inproceedings{lam2015multifidelity,
  title={Multifidelity optimization using statistical surrogate modeling for non-hierarchical information sources},
  author={Lam, R{\'e}mi and Allaire, Douglas L and Willcox, Karen E},
  booktitle={56th AIAA/ASCE/AHS/ASC Structures, Structural Dynamics, and Materials Conference},
  pages={0143},
  year={2015}
}



@article{kennedy2001bayesian,
  title={Bayesian calibration of computer models},
  author={Kennedy, Marc C and O'Hagan, Anthony},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={63},
  number={3},
  pages={425--464},
  year={2001},
  publisher={Wiley Online Library}
}



@article{olleak2020calibration,
  title={Calibration and validation framework for selective laser melting process based on multi-fidelity models and limited experiment data},
  author={Olleak, Alaa and Xi, Zhimin},
  journal={Journal of Mechanical Design},
  volume={142},
  number={8},
  pages={081701},
  year={2020},
  publisher={American Society of Mechanical Engineers}
}





@article{zhou2020generalized,
  title={A generalized hierarchical co-Kriging model for multi-fidelity data fusion},
  author={Zhou, Qi and Wu, Yuda and Guo, Zhendong and Hu, Jiexiang and Jin, Peng},
  journal={Structural and Multidisciplinary Optimization},
  volume={62},
  pages={1885--1904},
  year={2020},
  publisher={Springer}
}

@article{chen2023topsis,
  title={TOPSIS based multi-fidelity Co-Kriging for multiple response prediction of structures with uncertainties through real-time hybrid simulation},
  author={Chen, Cheng and Ran, Desheng and Yang, Yanlin and Hou, Hetao and Peng, Changle},
  journal={Engineering Structures},
  volume={280},
  pages={115734},
  year={2023},
  publisher={Elsevier}
}



@article{gardner2018gpytorch,
  title={Gpytorch: Blackbox matrix-matrix gaussian process inference with gpu acceleration},
  author={Gardner, Jacob and Pleiss, Geoff and Weinberger, Kilian Q and Bindel, David and Wilson, Andrew G},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@article{pof1,
  title={pBO-2GP-3B: A batch parallel known/unknown constrained Bayesian optimization with feasibility classification and its applications in computational fluid dynamics},
  author={Tran, Anh and Sun, Jing and Furlan, John M and Pagalthivarthi, Krishnan V and Visintainer, Robert J and Wang, Yan},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={347},
  pages={827--852},
  year={2019},
  publisher={Elsevier}
}


@inproceedings{csf1,
  title={Scalable constrained Bayesian optimization},
  author={Eriksson, David and Poloczek, Matthias},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={730--738},
  year={2021},
  organization={PMLR}
}

@article{csf2,
  title={BoTorch: A framework for efficient Monte-Carlo Bayesian optimization},
  author={Balandat, Maximilian and Karrer, Brian and Jiang, Daniel and Daulton, Samuel and Letham, Ben and Wilson, Andrew G and Bakshy, Eytan},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={21524--21538},
  year={2020}
}

@article{schonlau1998global,
  title={Global versus local search in constrained optimization of computer models},
  author={Schonlau, Matthias and Welch, William J and Jones, Donald R},
  journal={Lecture notes-monograph series},
  pages={11--25},
  year={1998},
  publisher={JSTOR}
}
@article{foumani2023multi,
  title={Multi-fidelity cost-aware Bayesian optimization},
  author={Foumani, Zahra Zanjani and Shishehbor, Mehdi and Yousefpour, Amin and Bostanabad, Ramin},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={407},
  pages={115937},
  year={2023},
  publisher={Elsevier}
}

@inproceedings{csf4,
  title={Bayesian optimization with inequality constraints.},
  author={Gardner, Jacob R and Kusner, Matt J and Xu, Zhixiang Eddie and Weinberger, Kilian Q and Cunningham, John P},
  booktitle={ICML},
  volume={2014},
  pages={937--945},
  year={2014}
}

@article{lin2023multi,
  title={A multi-objective bayesian optimization approach based on variable-fidelity multi-output metamodeling},
  author={Lin, Quan and Zheng, Anran and Hu, Jiexiang and Shu, Leshi and Zhou, Qi},
  journal={Structural and Multidisciplinary Optimization},
  volume={66},
  number={5},
  pages={100},
  year={2023},
  publisher={Springer}
}

@inproceedings{tran2019sbf,
  title={sBF-BO-2CoGP: A sequential bi-fidelity constrained Bayesian optimization for design applications},
  author={Tran, Anh and Wildey, Tim and McCann, Scott},
  booktitle={International Design Engineering Technical Conferences and Computers and Information in Engineering Conference},
  volume={59179},
  pages={V001T02A073},
  year={2019},
  organization={American Society of Mechanical Engineers}
}



@article{ur2017expected,
  title={Expected improvement based infill sampling for global robust optimization of constrained problems},
  author={ur Rehman, Samee and Langelaar, Matthijs},
  journal={Optimization and Engineering},
  volume={18},
  pages={723--753},
  year={2017},
  publisher={Springer}
}

@article{tran2022aphbo,
  title={aphBO-2GP-3B: a budgeted asynchronous parallel multi-acquisition functions for constrained Bayesian optimization on high-performing computing architecture},
  author={Tran, Anh and Eldred, Mike and Wildey, Tim and McCann, Scott and Sun, Jing and Visintainer, Robert J},
  journal={Structural and Multidisciplinary Optimization},
  volume={65},
  number={4},
  pages={132},
  year={2022},
  publisher={Springer}
}

@article{zanjani2024safeguarding,
  title={Safeguarding Multi-fidelity Bayesian Optimization Against Large Model Form Errors and Heterogeneous Noise},
  author={Zanjani Foumani, Zahra and Yousefpour, Amin and Shishehbor, Mehdi and Bostanabad, Ramin},
  journal={Journal of Mechanical Design},
  volume={146},
  number={6},
  year={2024},
  publisher={American Society of Mechanical Engineers Digital Collection}
}

@article{zhou2024multi,
  title={A multi-fidelity Bayesian optimization approach for constrained multi-objective optimization problems},
  author={Zhou, Qi and Shu, Leshi and Zhang, Anfu},
  journal={Journal of Mechanical Design},
  volume={146},
  pages={071702--1},
  year={2024}
}

@article{he2022variable,
  title={Variable-fidelity hypervolume-based expected improvement criteria for multi-objective efficient global optimization of expensive functions},
  author={He, Youwei and Sun, Jinju and Song, Peng and Wang, Xuesong},
  journal={Engineering with Computers},
  volume={38},
  number={4},
  pages={3663--3689},
  year={2022},
  publisher={Springer}
}



@article{berkenkamp2023bayesian,
  title={Bayesian optimization with safety constraints: safe and automatic parameter tuning in robotics},
  author={Berkenkamp, Felix and Krause, Andreas and Schoellig, Angela P},
  journal={Machine Learning},
  volume={112},
  number={10},
  pages={3713--3747},
  year={2023},
  publisher={Springer}
}

@inproceedings{wang2024constrained,
  title={Constrained Bayesian optimization under partial observations: Balanced improvements and provable convergence},
  author={Wang, Shengbo and Li, Ke},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={38},
  number={14},
  pages={15607--15615},
  year={2024}
}

@article{folch2024transition,
  title={Transition Constrained Bayesian Optimization via Markov Decision Processes},
  author={Folch, Jose Pablo and Tsay, Calvin and Lee, Robert M and Shafei, Behrang and Ormaniec, Weronika and Krause, Andreas and van der Wilk, Mark and Misener, Ruth and Mutn{\`y}, Mojm{\'\i}r},
  journal={arXiv preprint arXiv:2402.08406},
  year={2024}
}



@article{shi2020multi,
  title={Multi-fidelity modeling and adaptive co-kriging-based optimization for all-electric geostationary orbit satellite systems},
  author={Shi, Renhe and Liu, Li and Long, Teng and Wu, Yufei and Gary Wang, G},
  journal={Journal of Mechanical Design},
  volume={142},
  number={2},
  pages={021404},
  year={2020},
  publisher={American Society of Mechanical Engineers}
}

@article{tian2024boundary,
  title={Boundary Exploration for Bayesian Optimization With Unknown Physical Constraints},
  author={Tian, Yunsheng and Zuniga, Ane and Zhang, Xinwei and D{\"u}rholt, Johannes P and Das, Payel and Chen, Jie and Matusik, Wojciech and Lukovi{\'c}, Mina Konakovi{\'c}},
  journal={arXiv preprint arXiv:2402.07692},
  year={2024}
}

@article{krishnamoorthy2024eccbo,
  title={ECCBO: An Inherently Safe Bayesian Optimization with Embedded Constraint Control for Real-Time Optimization},
  author={Krishnamoorthy, Dinesh},
  journal={arXiv preprint arXiv:2402.18415},
  year={2024}
}

@article{tfaily2024bayesian,
  title={Bayesian optimization with hidden constraints for aircraft design},
  author={Tfaily, Ali and Diouane, Youssef and Bartoli, Nathalie and Kokkolaras, Michael},
  journal={Structural and Multidisciplinary Optimization},
  volume={67},
  number={7},
  pages={123},
  year={2024},
  publisher={Springer}
}

@article{gp+,
  title={GP+: a python library for kernel-based learning via Gaussian Processes},
  author={Yousefpour, Amin and Foumani, Zahra Zanjani and Shishehbor, Mehdi and Mora, Carlos and Bostanabad, Ramin},
  journal={Advances in Engineering Software},
  volume={195},
  pages={103686},
  year={2024},
  publisher={Elsevier}
}

@article{bostanabad2018leveraging,
  title={Leveraging the nugget parameter for efficient Gaussian process modeling},
  author={Bostanabad, Ramin and Kearney, Tucker and Tao, Siyu and Apley, Daniel W and Chen, Wei},
  journal={International journal for numerical methods in engineering},
  volume={114},
  number={5},
  pages={501--516},
  year={2018},
  publisher={Wiley Online Library}
}


@article{griffiths2020constrained,
  title={Constrained Bayesian optimization for automatic chemical design using variational autoencoders},
  author={Griffiths, Ryan-Rhys and Hern{\'a}ndez-Lobato, Jos{\'e} Miguel},
  journal={Chemical science},
  volume={11},
  number={2},
  pages={577--586},
  year={2020},
  publisher={Royal Society of Chemistry}
}

@article{sorourifar2021data,
  title={A data-driven automatic tuning method for MPC under uncertainty using constrained Bayesian optimization},
  author={Sorourifar, Farshud and Makrygirgos, Georgios and Mesbah, Ali and Paulson, Joel A},
  journal={IFAC-PapersOnLine},
  volume={54},
  number={3},
  pages={243--250},
  year={2021},
  publisher={Elsevier}
}

@article{letham2019constrained,
  title={Constrained Bayesian optimization with noisy experiments},
  author={Letham, Benjamin and Karrer, Brian and Ottoni, Guilherme and Bakshy, Eytan},
  year={2019}
}


@article{di2023nm,
  title={Nm-mf: Non-myopic multifidelity framework for constrained multi-regime aerodynamic optimization},
  author={Di Fiore, Francesco and Mainini, Laura},
  journal={AIAA Journal},
  volume={61},
  number={3},
  pages={1270--1280},
  year={2023},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{sorourifar2023computationally,
  title={Computationally efficient integrated design and predictive control of flexible energy systems using multi-fidelity simulation-based Bayesian optimization},
  author={Sorourifar, Farshud and Choksi, Naitik and Paulson, Joel A},
  journal={Optimal Control Applications and Methods},
  volume={44},
  number={2},
  pages={549--576},
  year={2023},
  publisher={Wiley Online Library}
}

@article{he2022batched,
  title={A batched bayesian optimization approach for analog circuit synthesis via multi-fidelity modeling},
  author={He, Biao and Zhang, Shuhan and Wang, Yifan and Gao, Tianning and Yang, Fan and Yan, Changhao and Zhou, Dian and Bi, Zhaori and Zeng, Xuan},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={42},
  number={2},
  pages={347--359},
  year={2022},
  publisher={IEEE}
}



@article{mathern2021multi,
  title={Multi-objective constrained Bayesian optimization for structural design},
  author={Mathern, Alexandre and Steinholtz, Olof Skogby and Sj{\"o}berg, Anders and {\"O}nnheim, Magnus and Ek, Kristine and Rempling, Rasmus and Gustavsson, Emil and Jirstrand, Mats},
  journal={Structural and Multidisciplinary Optimization},
  volume={63},
  pages={689--701},
  year={2021},
  publisher={Springer}
}

@article{ghoreishi2019multi,
  title={Multi-information source constrained Bayesian optimization},
  author={Ghoreishi, Seyede Fatemeh and Allaire, Douglas},
  journal={Structural and Multidisciplinary Optimization},
  volume={59},
  pages={977--991},
  year={2019},
  publisher={Springer}
}

@article{khatamsaz2023bayesian,
  title={Bayesian optimization with active learning of design constraints using an entropy-based approach},
  author={Khatamsaz, Danial and Vela, Brent and Singh, Prashant and Johnson, Duane D and Allaire, Douglas and Arr{\'o}yave, Raymundo},
  journal={npj Computational Materials},
  volume={9},
  number={1},
  pages={49},
  year={2023},
  publisher={Nature Publishing Group UK London}
}


@article{eweis2022data,
  title={Data fusion with latent map Gaussian processes},
  author={Eweis-Labolle, Jonathan Tammer and Oune, Nicholas and Bostanabad, Ramin},
  journal={Journal of Mechanical Design},
  volume={144},
  number={9},
  pages={091703},
  year={2022},
  publisher={American Society of Mechanical Engineers}
}

@article{zhang2018variable,
  title={Variable-fidelity expected improvement method for efficient global optimization of expensive functions},
  author={Zhang, Yu and Han, Zhong-Hua and Zhang, Ke-Shi},
  journal={Structural and Multidisciplinary Optimization},
  volume={58},
  pages={1431--1451},
  year={2018},
  publisher={Springer}
}


@inproceedings{saputro2017limited,
  title={Limited memory Broyden-Fletcher-Goldfarb-Shanno (L-BFGS) method for the parameter estimation on geographically weighted ordinal logistic regression model (GWOLR)},
  author={Saputro, Dewi Retno Sari and Widyaningsih, Purnami},
  booktitle={AIP conference proceedings},
  volume={1868},
  number={1},
  year={2017},
  organization={AIP Publishing}
}

@article{oune2021latent,
  title={Latent map Gaussian processes for mixed variable metamodeling},
  author={Oune, Nicholas and Bostanabad, Ramin},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={387},
  pages={114128},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{mohammed2017over,
  title={Over-fitting in model selection with Gaussian process regression},
  author={Mohammed, Rekar O and Cawley, Gavin C},
  booktitle={Machine Learning and Data Mining in Pattern Recognition: 13th International Conference, MLDM 2017, New York, NY, USA, July 15-20, 2017, Proceedings 13},
  pages={192--205},
  year={2017},
  organization={Springer}
}

@article{bracher2021evaluating,
  title={Evaluating epidemic forecasts in an interval format},
  author={Bracher, Johannes and Ray, Evan L and Gneiting, Tilmann and Reich, Nicholas G},
  journal={PLoS computational biology},
  volume={17},
  number={2},
  pages={e1008618},
  year={2021},
  publisher={Public Library of Science San Francisco, CA USA}
}



@misc{gp_plus,
  author       = {Bostanabad Research Group},
  title        = {GP-Plus: Examples},
  year         = {2025},
  url          = {https://github.com/Bostanabad-Research-Group/GP-Plus/tree/main/Examples},
  note         = {Accessed: 2025-01-24}
}


@article{moslemi2023scaling,
  title={Bayesian Parameter Inference and Uncertainty Quantification for a Computational Pulmonary Hemodynamics Model Using Gaussian Processes},
  author={Kachabi, Amirreza and Correa, Sofia Altieri and Chesler, Naomi C and Colebank, Mitchel J},
  journal={arXiv preprint arXiv:2502.14251},
  year={2025}
}


@article{ghorbanian2024empowering,
  title={Empowering approximate Bayesian neural networks with functional priors through anchored ensembling for mechanics surrogate modeling applications},
  author={Ghorbanian, Javad and Casaprima, Nicholas and Olivier, Audrey},
  journal={Computer Methods in Applied Mechanics and Engineering},
  pages={117645},
  year={2024},
  publisher={Elsevier}
}




























